Putting Them under Microscope: A Fine-Grained Approach for Detecting Redundant Test Cases in Natural Language

Natural language (NL) documentation is the bridge between software managers and testers, and NL test cases are prevalent in system-level testing and other quality assurance activities. Due to reasons such as requirements redundancy, parallel testing, and tester turnover within long evolving history, there are inevitably lots of redundant test cases, which significantly increase the cost. Previous redundancy detection approaches typically treat the textual descriptions as a whole to compare their similarity and suffer from low precision. Our observation reveals that a test case can have explicit test-oriented entities, such as tested function Components, Constraints, etc; and there are also specific relations between these entities. This inspires us with a potential opportunity for accurate redundancy detection. In this paper, we first define five test-oriented entity categories and four associated relation categories and re-formulate the NL test case redundancy detection problem as the comparison of detailed testing content guided by the test-oriented entities and relations. Following that, we propose Tscope, a fine-grained approach for redundant NL test case detection by dissecting test cases into atomic test tuple(s) with the entities restricted by associated relations. To serve as the test case dissection, Tscope designs a context-aware model for the automatic entity and relation extraction. Evaluation on 3,467 test cases from ten projects shows Tscope could achieve 91.8% precision, 74.8% recall, and 82.4% F1, significantly outperforming state-of-the-art approaches and commonly-used classifiers. This new formulation of the NL test case redundant detection problem can motivate the follow-up studies to further improve this task and other related tasks involving NL descriptions.

==> sec/3.background.tex <==
\section{Empirical analysis of entity categories for redundancy detection}
\label{sec:background}
This section introduces test redundancy in practice and the joint extraction model for entity and relation extraction in NLP field.

\subsection{Test Case Redundancy in Practice}
\label{background:redundancy}
% 说一下测试用例之间冗余是怎么产生的，主要结合practical selective regression testing with effective redundancy in interleaved test这篇文章2.1章节改写一下，也结合一下2.1章节引用的【6】这篇论文。
% 主要是阐述之前你做ppt给王老师讲过的那个产生冗余的原因，用2-3段写几个你能解释地清楚的原因即可。
% \begin{figure}[htbp]
% \centering
% \includegraphics[width=\columnwidth]{fig/testcase_redundant.eps}
% \caption{Reasons for generating redundant test cases}
% \label{fig:testcase_redundancy}
% \end{figure}

Test case redundancy is a common problem in practice, and has been studies for a long time in the literature.
According to previous study, there are many reasons for redundant test cases, such as incomplete requirements specification, parallel testing, distributed testing, testing in generic area, legacy systems and so on \cite{engstrom2013test}. 
In our practice, we observe that redundant test cases produce mainly due to the redundancy of requirements.
Specifically, in the testing phrase, testing engineers analyze each requirement, identify all the test execution scenarios and instantiate them in test cases.
A requirement covers multiple features, and there may be overlapping features among requirements.
For a large software project, the requirements are typically tested by different test engineers, and test engineers are not aware of the feature overlapping.
Test redundancy may produce when each test engineer individually designs test case(s) for assigned requirements.

Another scenario is that overlapping features between new requirements and implemented requirements when software evolves. 
In this case, test engineers are not aware that some test cases could be reused for the new requirements, and redesign test cases for the implemented requirements.
When the new test cases are added into the test suite for the software project, the redundancy produces.

As reported by previous studies, redundant test cases have resulted in a large amount of testing cost and maintenance effort as the system evolves and test suite grows \cite{jeffrey2005test,fraser2007redundancy,hooda2018test}.
According to investigation of our industrial partner, there are no less than 25\% test cases are redundant in their test suite, which significantly affect the test efficiency in practice.
Our approach aims at automatically detecting redundant test cases to reduce the testing cost for our industrial partner.

% Test case redundancy is usually defined in terms of coverage metrics \cite{marijan2018practical}. Taking pairwise feature coverage in coverage strategies as an example, if two test cases execute the same pairwise feature, one of the two test cases is considered redundant.

% In our project, the reason for redundant test cases is the redundancy between requirements. As shown in Figure \ref{fig:testcase_redundancy}, the left half of the figure shows the requirements of the basic editing functions of graphics, and the right half is the requirements for the color adjustment of the graphics. The same functionality exists between the two requirements, so there is a redundant relation between the test cases designed for the two requirements. For example, test case 346 in
% figure \ref{fig:testcase_redundancy} is redundant with test case 525 and test case 526, respectively.


% We summarize the reasons for test case redundancy into the following categories: (1) Redundancy in requirements: The different granularity of requirement description described by user stories leads to redundancy among different requirements, so the derived test cases are also redundant. (2) Integration Testing: due to negligence in designing test cases, different test cases contain the same characteristics, and integrating such test cases will result in the execution of the same function in multiple instances. (3) System testing of generic areas: Common areas between different systems will have a lot of duplicate functions, and when the systems are integrated, redundant test cases will be generated. (4) Parallel testing: At the same time, the same test cases are tested on different branches, resulting in redundant test cases.



 
\subsection{Entity and Relation Extraction in NLP}
\label{sec:relatad_extraction}
%说一下传统的单独ENtity 和Relation抽取的做法，然后说有错误累计的问题；
%然后说一下最新的做法都是joint extraction；
% 说一下joint extraction的一般流程，比如先说embedding，然后是entity classification，然后是relation classification；
% 最后说一下，我们也是引用了联合抽取的模型，抽取关键元素进行比较；

\begin{figure}[tbh]
% \begin{centerline}
% \includegraphics[width=\textwidth]{architechture.eps}
\begin{center}
  \includegraphics[height=4cm,width=8.5cm]{fig/traditional_extractmodel.png}
  \end{center}
    \caption{
     The general framework of joint extraction model
    }
    \label{fig:traditional_model}    
% \end{centerline}
\end{figure}

Traditional deep learning supervised entity relation extraction adopts pipeline method \cite{zheng2017joint}.  The traditional pipelined methods divide the task into two independent sub-tasks, namely named entity recognition (NER) task \cite{nadeau2007survey}, and relation classification task \cite{rink2010utd}, then design methods to solve these two sub-tasks respectively. The traditional pipelining makes tasks easier to handle and each component can be more flexible. But it ignores the dependencies of the two subtasks. The results of entity recognition may affect the performance of relation classification and lead to erroneous delivery. Compared with the pipeline method, the joint learning method \cite{zheng2016joint} can utilize the close interaction information between entities and relations, extract entities and classify the relationship of entity pairs at the same time, and solve the problems existing in the pipeline method. The general framework of joint extraction model is shown in Figure \ref{fig:traditional_model}. The input of the entity classification component is the hidden state representation of the entity, and the input of the relation classification component is the candidate entity pair. The two components are jointly trained with Loss parameters to realize the information interaction between entities and relations. In this paper, we introduce the joint extraction model to extract significant elements in test cases, which contribute to identify redundant relations between test cases.


==> sec/camera-ready_revisions.tex <==
1.基线文字描述错误更正；(已修改)
2.discussion中测试用例依赖图中的语法错误更正；（学长figure 6的原图发我下）
3.数据集的描述表达清晰；(在2.2节添加了脚注)
4.Performance Measurement添加到RQ1、RQ2； (已添加)
5.Section2中加一下实体、关系构建的过程描述；
6.作者信息；
7.致谢信息；
8.比较策略中描述的词性信息弱化一些？？？
9.给个测试用例的例子？？？

Github代码有点乱  （已调整）

==> sec/todo.tex <==
TODO LIST：
    1. 方法图更新--------已完成；
    2. 模型图更新--------已完成；
    3. background改写--------已完成；
    % 4. 背景中实体和关系联合抽取简介--------已完成：
    %     a. 需要画图说明基本结构；
    %     b. 是否要放到related work？？？
    5. RQ1结果分析；
    6. 实体关系类的两个表，更新，记得加个缩写！--------已完成
    7. 给方法和抽取模型取个名；
    % 8. Abstract和Introduction中实验结果要加上RQ1的结果;
    9. 方法部分有一个overview还没有写--------已完成;
    10. SIF加引用--------已完成；
    11. Cosine相似度加引用--------已完成；
    12. 方法部分是否需要加一个例子来说明实体和关系的标注；
    13. 方法的可解释性是否可以加入discussion？？？？（空间多余时再写）
    14. 相似度阈值还没描述；--------已完成
    15. span长度还没描述；--------已完成
    16. Reference大于50；
    17. results部分加summary（空间多余时再写）
    


Checking List before submitting：
    1. entity category and relation entity的简写是否正确，全文检查；
    2. 1-10的数字全部改成 one two three... ten，全文检查；
    3. 表名称、标题名称中不要有.，全文检查；
    4. ref cite是否有???；
    5. preciison和recall的大小写统一，都统一到Precision Recall F1；
    6. 性能表述时用\%表述，保留一位小数
    7. 标题、表名、图片名的大小写格式；
    8. 
    
    
TODO LIST 20220308
1. 相关性分析结果放到表里面； --------已完成;
2. 方法名最后一个步骤 detecting redundant test cases换个名，指向性更明确一些； （Redundant test case identification）
3. 方法中model construction 没有蓝色的步骤；
4. 模型图中V4、V5、V1换成黄色； --------已完成
5. CLS要不要写（和C0、C1一起当做上下文信息）---再讨论；
6. RQ2的图中监督学习的方法---再讨论；
7. Table5删了，对应的文字修改；--------已完成
8. Dataset 说一下来自4个厂家的10个操作系统产品；--------已完成
9. Non-redundancy考虑一下RQ2、RQ3; --------已完成（RQ3考虑不加）
10. 6.2删了，改成说明如何利用5个类写好测试用例。  (目前加完9中的表和文字，基本就没有空间再加这一部分)
11.名称现在考虑叫TEAM ：	TEst cAses Microscope Redundancy

==> tab/extract_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
 \caption{The Performance of {\extraction}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textit{\textbf{Approach}}}} & \multicolumn{3}{c|}{\textbf{Entity}}                                             & \multicolumn{3}{c|}{\textbf{Relation}}                                                           \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Recall}}  & \textbf{F1}      & \multicolumn{1}{l|}{\textbf{Precision}} & \multicolumn{1}{l|}{\textbf{Recall}}  & \textbf{F1} \\ \hline
Our                                             & \multicolumn{1}{c|}{96.4\%}    & \multicolumn{1}{c|}{94.76\%} & 95.38\% & \multicolumn{1}{c|}{89.59\%}   & \multicolumn{1}{c|}{97.85\%} & 93.38\%                 \\ \hline
Baseline                                        & \multicolumn{1}{c|}{92.12\%}   & \multicolumn{1}{c|}{92.88\%} & 91.9\%  & \multicolumn{1}{c|}{77.31\%}   & \multicolumn{1}{c|}{96.64\%} & 85.48\%                 \\ \hline
\end{tabular}
}
\label{tab:extract_model}
\end{table}

==> tab/project_nonredundancy.tex <==
\begin{table}[htbp]

\caption{The Non-redundant detection performance}
\label{tab:non-redundancy_project}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule
{\textbf{Project}} & {\textbf{NonR\_Precision}} & {\textbf{NonR\_Recall}} & {\textbf{NonR\_F1}} \\ \midrule
1                                    & 91.06\%                                   & 98.19\%                                & 94.49\%                            \\
2                                    & 81.53\%                                   & 95.78\%                                & 88.08\%                            \\
3                                    & 89.38\%                                   & 96.38\%                                & 92.75\%                            \\
4                                    & 81.25\%                                   & 96.02\%                                & 88.02\%                            \\
5                                    & 86.74\%                                   & 96.01\%                                & 91.13\%                            \\
6                                    & 79.16\%                                   & 93.95\%                                & 85.92\%                            \\
7                                    & 90.62\%                                   & 96.66\%                                & 93.54\%                            \\
8                                    & 88.58\%                                   & 96.15\%                                & 92.21\%                            \\
9                                    & 84.15\%                                   & 94.84\%                                & 89.17\%                            \\
10                                   & 80.67\%                                   & 93.29\%                                & 86.52\%                            \\ \midrule
\textbf{Average}                     & \textbf{85.31\%}                          & \textbf{95.72\%}                       & \textbf{90.18\%}                   \\ \bottomrule
\end{tabular}
}
\end{table}

==> tab/project_redundancyperformance.tex <==
\begin{table}[htbp]

\caption{The Non-redundant detection performance for each project}
\label{tab:redundancy_project}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ c c c c c c }
\toprule
\multicolumn{1}{ l }{\textbf{Project}} & \multicolumn{1}{l }{\textbf{R\_precision}} & \multicolumn{1}{l }{\textbf{R\_recall}} & \multicolumn{1}{l }{\textbf{R\_F1}} & \multicolumn{1}{l }{\textbf{Redundant TCs}} & \multicolumn{1}{l }{\textbf{Total TCs}} \\ \midrule
1                                      & 94.23\%                                    & 75.38\%                                 & 83.76\%                             & 52                                         & 220                                    \\ 
2                                      & 94.65\%                                    & 77.5\%                                 & 85.23\%                             & 59                                         & 232                                    \\ 
3                                      & 89.28\%                                    & 72.46\%                                 & 80.00\%                             & 56                                          & 227                                    \\ 
4                                      & 94.85\%                                    & 76.78\%                                  & 84.86\%                             & 59                                         & 234                                    \\ 
5                                      & 91.17\%                                    & 73.81\%                                 & 81.57\%                              & 68                                          & 234                                    \\ 
6                                      & 91.79\%                                     & 73.21\%                                 & 81.45\%                             & 41                                          & 221                                    \\ 
7                                      & 93.05\%                                    & 81.7\%                                 & 87.01\%                             & 72                                          & 232                                    \\ 
8                                      & 89.53\%                                     & 72.64\%                                 & 80.2\%                             & 74                                         & 239                                    \\ 
9                                      & 89.25\%                                     & 70.58\%                                 & 78.83\%                             & 70                                         & 236                                    \\ 
10                                     & 89.74\%                                    & 72.41\%                                 & 80.15\%                             & 50                                         & 222                                    \\ \midrule
\textbf{Average}                       & \textbf{85.31\%}                           & \textbf{95.72\%}                        & \textbf{90.18\%}                    & \textbf{60}                                 & \textbf{230}                                     \\ \bottomrule
\end{tabular}
}

\end{table}

==> tab/relation_category.tex <==
\begin{table}[htbp]
\large
  \caption{Description of Relation Categories}
  \label{tab:relation_category}
\resizebox{0.8\columnwidth}{!}{
  \begin{tabular}{cc}
    \toprule
     \textbf{Relation Entity} & \textbf{Associated Entities} \\   
      \midrule
    Acts  &   \textit{Component} -> \textit{Behavior} \\
    Exists &  \textit{Component} -> \textit{State}\\ 
    Assists &   \textit{Component} -> \textit{Means} \\
    Satisfies &  \textit{Component} -> \textit{Standard} \\
    \bottomrule
  \end{tabular}
}
\end{table}

==> tab/tuple_exampleold.tex <==
\begin{table}[htbp]
\large
  \caption{Tuples Decomposed from Test Case \#346 and \#525}
  \label{tab:tuplesold}
\resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccccc}
    \toprule
     \textbf{Test Case} &   \textbf{Tuple} & \textbf{Component} & \textbf{Behavior}& \textbf{State}& \textbf{Means}& \textbf{Condition}\\   
      \midrule
~   &   Tuple-1  &  point    &   draw    &   NULL    &   drawing editor &   NULL\\
\#346   &   Tuple-2 &   line    &   draw    &   NULL    &   drawing editor &   NULL   \\ 
~   &   Tuple-3 &   rectangle    &   draw    &   NULL    &   drawing editor &   NULL\\
~   &   Tuple-4 &   image color   &   adjust    &   NULL    &   drawing editor &   NULL\\
\midrule
~   &   Tuple-5  &  point    &   draw    &   NULL    &   drawing editor &   NULL\\
\#525   &   Tuple-6 &   line    &   draw    &   NULL    &   drawing editor &   NULL   \\ 
~   &   Tuple-7 &   rectangle    &   draw    &   NULL    &   drawing editor &   NULL\\

    \bottomrule
  \end{tabular}
}
\end{table}
